Sensor Transfer: Learning Optimal Sensor Effect Image Augmentation for Sim-to-Real Domain Adaptation

Performance on benchmark datasets has drastically improved with advances in deep learning. Still, cross-dataset generalization performance remains relatively low due to the domain shift that can occur between two different datasets. This domain shift is especially exaggerated between synthetic and real datasets. Significant research has been done to reduce this gap, specifically via modeling variation in the spatial layout of a scene, such as occlusions, and scene environmental factors, such as time of day and weather effects. However, few works have addressed modeling the variation in the sensor domain as a means of reducing the synthetic to real domain gap. The camera or sensor used to capture a dataset introduces artifacts into the image data that are unique to the sensor model, suggesting that sensor effects may also contribute to domain shift. To address this, we propose a learned augmentation network composed of physically-based augmentation functions. Our proposed augmentation pipeline transfers specific effects of the sensor model -- chromatic aberration, blur, exposure, noise, and color temperature -- from a real dataset to a synthetic dataset. We provide experiments that demonstrate that augmenting synthetic training datasets with the proposed learned augmentation framework reduces the domain gap between synthetic and real domains for object detection in urban driving scenes.

==> askc_abstract.tex <==
%%
Performance on benchmark datasets has drastically improved with advances in deep learning. Still, cross-dataset generalization performance remains relatively low due to the domain shift that can occur between two different datasets. This domain shift is especially exaggerated between synthetic and real datasets. %, especially for visual tasks in urban driving scenes. 
%This problem of domain shift is particularly bad for training on synthetic datasets and testing in the real domain.
%
%In an effort to mitigate synthetic to real domain shift, 
Significant research has been done to reduce this gap, 
%specifically in generating synthetic data that better captures the variation of real training datasets,
specifically via modeling variation in the spatial layout of a scene, such as occlusions, and scene environmental factors, such as time of day and weather effects. 
%
However, few works have addressed modeling the variation in the sensor domain as a means of reducing the synthetic to real domain gap. 
The camera or sensor used to capture a dataset introduces artifacts into the image data that are unique to the sensor model, suggesting that sensor effects may also contribute to domain shift. 
%We show that the distribution over these photometric effects is different across vehicle benchmark datasets for both real and synthetic data, and that differences in the representation of sensor effects in captured data contributes to domain shift between datasets. 
To address this, we propose a learned augmentation network composed of physically-based augmentation functions. Our proposed augmentation pipeline transfers specific effects of the sensor model -- chromatic aberration, blur, exposure, noise, and color temperature -- from a real dataset to a synthetic dataset. 
%We provide experiments that demonstrate that augmentation of synthetic training images with sensor effects improves the robustness and generalizability of object detection networks trained in the reaon benchmark vehicle datasets.
We provide experiments that demonstrate that augmenting synthetic training datasets with the proposed learned augmentation framework reduces the domain gap between synthetic and real domains for object detection in urban driving scenes.

%Recent work has focused on generating synthetic imagery to increase the size and variability of training data for learning visual tasks in urban scenes. This includes increasing the occurrence of occlusions or varying environmental and weather effects. 
%However, few have addressed modeling variation in the sensor domain. 
%Unfortunately, sensor effects can degrade performance and generalizability of neural network performance for visual tasks trained on human annotated datasets. 
%Sensor effects can degrade real images, limiting generalizability of network performance on visual tasks trained on synthetic data and tested in real environments. 
%This paper proposes an efficient, automatic, physically-based augmentation pipeline to vary sensor effects -- chromatic aberration, blur, exposure, noise, and color temperature -- for synthetic imagery. 
%In particular, this paper illustrates that augmenting synthetic training datasets with the proposed framework reduces the domain gap between synthetic and real domains for the tasks of object detection and semantic segmentation in urban driving scenes. 



==> askc_background.tex <==
%% BACKGROUND
%
Our work focuses on augmenting the training data directly so that it can be applied to any task or input into any deep neural network regardless of the architecture. 
Zhang et al. 2017~\cite{zhang2017physically} demonstrate that the level of photorealism of the synthetic training data directly impacts the robustness and performance of the deep learning algorithm when tested on real data across a variety of computer vision tasks. However, it remains unclear what features of real data are necessary for this performance gain, or what parts of rendering pipelines should be modified to bridge the synthetic to real domain gap. 
Much work in the fields of data augmentation and learned rendering pipelines have proposed methods that shed light on  this topic, and are summarized below. 
%% Synthetic
%\vspace{-5mm}
%\subsection{Synthetic Datasets} 
%Rendering and gaming engines have been used to synthesize datasets that contain a wide variety of environmental factors that could not be feasibly captured during real data collection. Such factors include time of day, weather, and community. architecture~\cite{gaidon2016virtual}~\cite{ros2016synthia}
%While improvements to rendering engines have focused on matching the photorealism of the generated data to real images, such photorealim comes at a huge computational cost. Consequently, synthetic datasets often contain visual artifacts from the rendering engine that do not exist in the real world, and thus do not capture the information in real images with high fidelity.
%Zhang et. al 2017 ~\cite{zhang2017physically} demonstrates that the level of photorealism of the synthetic training data directly impacts the robustness and performance of the deep learning algorithm when tested on real data across a variety of computer vision tasks. However, it remains unclear what features of real data are necessary for this performance gain, or what parts of the rendering pipelines should be modified to bridge the synthetic to real domain gap. 
%This evidenced by the fact that state-of-the art synthetic datasets need to be orders of magnitude larger than real datasets to achieve the same level of performance achieved when training on real data~\cite{johnson2017driving, ros2016synthia,tian2018training}, and often require fine-tuning on real data regardless.
%In comparison, our \textit{sensor tranfser} framework can be used to generate smaller sets of synthetic data that achieve higher performance that state-of-the-art photorealistic datasets.
%
\vspace{-2mm}
\subsection{Domain Randomization} 
%In contrast to focusing on altering the rendering pipeline/how synthetic images are generated, which can be unstable, 
%Rendering and gaming engines have been used to synthesize large, labelled datasets that contain a wide variety of environmental factors that could not be feasibly captured during real data collection~\cite{ros2016synthia,gaidon2016virtual} or that could not be feasibly rendered due to computational expense~\cite{tobin2017domain}. Such factors include time of day, weather, and community architecture. 
Recent work on domain randomization seeks to bridge the sim-to-real domain gap by generating synthetic data that has sufficient random variation over scene factors and rendering parameters such that the real data falls into this range of variation, even if the rendered data does not appear photorealistic. Such scene factors include such as textures, occlusion levels, scene lighting, camera field of view, and uniform noise, and have been applied to vision tasks in complex indoor and outdoor environments~\cite{tobin2017domain,tremblay2018training}. 
%%can be eliminated if the network is trained on synthetic data with sufficient enough (not necessarily realistic) variation/random environment pertubation such that 
%%Training on these datasets enables the network to learn invariance to visual features that are independent of real world scene factors that impact the appearance of objects in an image. 
%%Paulin et. al~\cite{paulin2014transformation} use validation accuracy during training to rank the importance of various augmentations, including flip, viewpoint changes, scale, RGB color jitter, JPEG compression, and rotations. These transformations are applied to both the training and testing data, so it is unclear from their results if these augmentations are in fact adding useful visual information for improving algorithm performance in the real data domain.
%Tobin et. al~\cite{tobin2017domain} focus on the task of object localization trained with synthetic data. They perform domain randomization over textures, occlusion levels, scene lighting, camera field of view, and uniform noise within the rendering engine, but their experiments are limited to highly simplistic toy scenes. %They explicitly state that they do not use physically realistic augmentation models for rendering. 
%Building on~\cite{tobin2017domain}, Tremblay et al~\cite{tremblay2018training} generate a synthetic dataset via domain randomization for object detection of real urban driving scenes. They randomize camera viewpoint, light source, object properties, and introduce flying distractors. 
%Our work focuses on image augmentation outside of the rendering pipeline and could be applied in addition to domain randomization in the renderer.
%SceneNet RGB-D: 5M Photorealistic Images of Synthetic Indoor Trajectories with Ground Truth renders dataset using domain randomization???
The drawback of these techniques is that they only work if they sample the visual parameters spaces finely enough, and create a large enough dataset from a broad enough range of visual distortions to encompass the variation observed in real data. This can result in intractably large datasets that require significant training time for a deep learning algorithm.
While we also aim to achieve robustness via an augmentation framework, we can use smaller datasets to achieve state-of-the-art performance because our method is learning how to augment synthetic data with salient visual information that exists in real data.
Note that, because our work focuses on image augmentation outside of the rendering pipeline, it could be used in addition to domain randomization techniques.
%
\vspace{-2mm}
\subsection{Optimizing Augmentation}
In contrast to domain randomization, task-dependent techniques have been proposed to achieve more efficient data augmentation by learning the type and number of image augmentations that are important for algorithm performance.
%Lemly et. al uses task performance to guide image blending augmentation for classification tasks ~\cite{lemley2017smart}.
%Cubuk et. al~\cite{cubuk2018autoaugment} use a reinforcement learning search algorithm to select an optimal data augmentation policy from a variety of standard augmentations, including spatial manipulations like rotation, shearing and inverting augmentations, and photometric manipulations like brightness, contrast, and color.
%Paulin et. al~\cite{paulin2014transformation} use validation accuracy during training to rank the importance of various augmentations, including flip, viewpoint changes, scale, RGB color jitter, JPEG compression, and rotations. 
%These transformations are applied to both the training and testing data, so it is unclear from their results if these augmentations are in fact adding useful visual information for improving algorithm performance in the real data domain.
State-of-the-art methods~\cite{paulin2014transformation,cubuk2018autoaugment,lemley2017smart} in this area treat data augmentation as a form of network regularization, selecting a subset of augmentations that optimize algorithm performance for a given dataset and task as the algorithm is being trained.
Unlike these methods, we propose that data augmentation can function as a domain adaptation method. Our learning framework is task-independent, and uses physically based augmentation techniques to investigate the visual degrees of freedom (defined by physically-based models) necessary for optimizing network performance from the synthetic to real domain. 
%Several studies have investigated manipulating images in a visually-realistic manner to improve neural network robustness. Eitel et al.~\cite{eitel2015multimodal} propose a physically-based data augmentation scheme specifically for depth images. They model realistic depth (Kinect) sensor noise as missing data patterns (i.e., occlusions and missing sensor data). In this study we focus on the more high-dimensional problem of modeling realistic sensor noise in RGB images.
%
%Unlike the above methods, which are similar to image-to-image translation methods~\cite{zhu2017unpaired} and can be unstable for high resolution imagery, our method can be applied to any image dataset. 
%Our approach also works on high resolution imagery. 
%We make this point to contrast our method with other methods, in particular generative networks and image-to-image translation methods, which may be unstable for higher resolution imagery.
%
%\vspace{-2mm}
% Deep Learning to improve rendering pipelines
%\subsection{Learned Rendering and Augmentation Pipelines for Synthetic Data:} 
%Several studies have proposed generative learning frameworks that take the place of a standard rendering engine or complement the rendering engine in order to learn the relevant visual information directly from real images. 
%Shrivastava et. al~\cite{simgan} recently developed SimGAN, a generative adversarial network (GAN) to augment synthetic data to appear more realistic. They evaluated their method on the the tasks of gaze estimation and hand pose estimation. 
%Similarly, Sixt et. al~\cite{sixt2016rendergan} proposed RenderGAN, a generative network that uses structured augmentation functions to augment synthetic images of markers attached to honeybees. The augmented images are used to train a detection network to track the honeybees. 
%Both of these approaches focus on image sets that are homogeneously structured and low resolution. We instead focus on the application of autonomous driving, which features highly varied, complex scenes and environmental conditions. 
%Veeravasarapu et. al~\cite{veeravasarapu2017adversarially} present an adversarial scene generation pipeline that renders synthetic scenes. They use their framework to learn distributions over light sources, weather patterns, and camera extrinsics from real data. 
%Huang et. al~\cite{huangexpecting} also propose an adversarial framework to learn a prior over model parameters for rendering synthetic pedestrians on natural images.
%Our work also focuses specifically on modeling the camera and image processing pipeline rather than scene elements or environmental factors that are specific to a given task.
%
%\vspace{-5mm}
%\subsection{Domain Transfer Methods for Sim-to-Real:}
%
%\subsubsection{Augmenting Neural Network Architecture}
%Recent work has focused on domain adaptation to improve accuracy in semantic segmentation of urban scenes~\cite{hoffmanfcnwild2016,sankaranarayanansynthiagan2017,hoffmanfcnwild2016,zhang2017curriculum} as well as object detection in urban environments~\cite{chen2018domain}. 
%These works alter the underlying network structure to shift the learned representation of the source and target datasets. 
%Our work instead focuses on augmenting the training data directly so that it can be applied to any task or input into any network regardless of the architecture.
%
\red{
%% added in response to reviewer 1's recommendation to add in citations and experiments for image-to-image translation methods
\subsection{Image-to-Image Translation for Domain Adaptation}
Impressive advances have been made in using both paired and unpaired image-to-image translation networks~\cite{CycleGAN2017,johnson2016perceptual,zhu2016generative,isola2017image,huang2018multimodal,liu2017unsupervised} to bridge a variety of domain gaps, including season-to-season, night-to-day, and sim-to-real.
While these methods have shown success in transferring the style of one real dataset to another with few to no constraints, results on transferring between image sets with complex, varied scenes often introduces artifacts to the image, which distorts the underlying structure of the scene, and thus can yeild poor performance for visual tasks such as object detection and semantic segmentation~\cite{dundar2018domain}. Furthermore, it is unclear if realistic, physically-based visual information is being transferred between domains (i.e, it is unclear that the image to image translation network actually learns a model of snow when transferring between season domains.
}

\subsection{Learned Rendering Pipelines for Domain Adaptation}
Several studies have proposed unsupervised, generative learning frameworks that either take the place of a standard rendering engine~\cite{veeravasarapu2017adversarially} or complement the rendering engine via post-processing~\cite{sixt2016rendergan,simgan,huangexpecting} in order to model relevant visual information directly from real images with no dependency on a specific task framework.  % or network architectures. 
%Shrivastava et. al~\cite{simgan} recently developed SimGAN, a generative adversarial network (GAN) that manipulates local pixel statistics in synthetic data to resemble the local structure in real images. They evaluated their method on the the tasks of gaze estimation and hand pose estimation for grayscale images.
%Similarly, Sixt et. al~\cite{sixt2016rendergan} proposed RenderGAN, a generative network that uses structured augmentation functions to manipulate synthetic images of markers attached to honeybees.  
%These methods can be divided into two areas. 
Both ~\cite{veeravasarapu2017adversarially} and ~\cite{huangexpecting} are applied to complex outdoor image datasets, but are designed to learn distributions over simpler spatial features in real images, specifically scene geometry. Other methods, such as ~\cite{sixt2016rendergan,simgan}, attempt to learn low-level pixel features. However, they are only applied to image sets that are homogeneously structured and low resolution. This may be due to the sensitivity of training adversarial frameworks. 
%However, many of these approaches focus on image sets that are homogeneously structured and low resolution, and can be unstable if applied to complex, high resolution datasets. 
%While our proposed method learns to model pixel statistics of real images, it does not use an adversarial loss, and is thus easily applied to datasets that feature highly varied, complex scenes, lighting, and environmental conditions, such as autonomous driving benchmarks. 
%Veeravasarapu et. al~\cite{veeravasarapu2017adversarially} present an adversarial scene generation pipeline that renders synthetic scenes. They use their framework to learn distributions over light sources, weather patterns, and camera extrinsics from real data. 
%Huang et. al~\cite{huangexpecting} also propose an adversarial framework to learn a prior over model parameters for rendering synthetic pedestrians on natural images.
Our work focuses specifically on modeling the camera and image processing pipeline rather than scene elements or environmental factors that are specific to a given task. Our method can be applied to high resolution images of complex scenes.
%
%\subsubsection{Image-to-image Translation}
%Advances have also been made in both paired and unpaired task-independent image-to-image translation networks~\cite{CycleGAN2017,johnson2016perceptual,zhu2016generative}. 
%While these methods have shown success in transferring the style of one real dataset to another with few to no constraints, results on transferring image sets with varied scene structure often introduces artifacts to the image, which distorts the underlying structure of the scene. 
%Dundar et. al 2018 ~\cite{dundar2018domain} propose a photorealistic style transfer algorithm that augments synthetic data better than the above GAN image to image translation methods for both semantic segmentation and object detection performance. Their method however relies on the labels associated with both the real and synthetic datasets. 
%In contrast, our method enacts physically-based manipulations in image space independent of the semantic labels or masks associated with each image. 
%We specifically model the camera effects of a particular dataset to achieve realistic and representative variation across photometric effects present in real data. Our method does not modify the underlying scene structure, style, or texture and thus does not introduce artifacts into the image.
%
%\vspace{-2mm}
% Sensor effects specific
\subsection{Impact of Sensor Effects on Deep Learning} 
%reference handa et al who uses realistic sensor noise models to augment depth data to improve pixel-level tasks
Recent work has demonstrated that elements of the image formation and processing pipeline can have a large impact upon learned representation for deep neural networks across a variety of vision tasks~\cite{Kanan2012,diamond2017dirty,dodge2016understanding,doersch2015unsupervised}. 
The majority of methods propose learning techniques that remove these effects from images~\cite{diamond2017dirty}. As many of these sensor effects can lead to loss of information, correcting for them is non-trivial, potentially unstable, and may result in the hallucination of visual structure in the restored image. 
%Other popular methods, some of which are described in above sections~\cite{lemley2017smart,huangexpecting,}, treat augmentation with such effects as simple forms of network regularization, and thus do not utilize realistic models. 
In contrast, Carlson et al.~\cite{carlson2018modeling} demonstrate that significant performance boosts can be achieved by augmenting images using physically-based, sensor effect domain randomization.
However, their method requires hand-tuning/evaluation of the visual quality of image augmentation. This human-in-the-loop dependence is inefficient and difficult to scale for large synthetic datasets, and the evaluated visual image quality is subjective.
%and entirely dependent upon the opinion of whoever is performing the evaluation/parameter selection. 
Rather than removing these effects, randomly adding them in, or manually adding them in via human-in-the-loop, our method learns the the style of sensor effects from real data and transfers this \textit{sensor style} to synthetic images to bridge the synthetic-to-real domain gap. 



==> tables/ST-numaug-objdet-table.tex <==
%%
\setlength{\tabcolsep}{1.0pt}
\begin{table*}
\begin{center}
%\caption{Object detection trained on synthetic data}
%\label{table:kittiandcityablation}
\caption{Results of the learned sensor effects augmentations on Faster R-CNN object detection performance. The percent change for both the Hand-tuned and Sensor-transfer Augmentations are calculated relative to the full, unaugmented baseline datasets.}
\label{table:numaug_results}
\begin{tabular}{cccc}
\begin{tabular}{|l|llllllllll|}
%\hline
%\noalign{\smallskip}
\multicolumn{5}{c}{Training Dataset} & \multicolumn{5}{c}{Tested on KITTI}   \\
\hline
%\noalign{\smallskip}
Augmentation Method       &&&&& $AP_{Car}$ &&&&& \footnotesize{Gain} \\
%\noalign{\smallskip}
\hline
%\noalign{\smallskip}
GTA\textit{Sim10k} Baseline                                            &&&&& 51.01 &&&&& \textemdash\\  
\scriptsize{Sensor Effect Dom. Rand. 10k unaug. + 2k aug.}             &&&&& 48.94 &&&&& $\downarrow$2.07 \\ 
\scriptsize{Sensor Effect Dom. Rand. 10k unaug. + 5k aug.}             &&&&& 48.52 &&&&& $\downarrow$2.49 \\
\scriptsize{Sensor Effect Dom. Rand. 10k unaug. + 8k aug.}             &&&&& 46.35 &&&&& $\downarrow$4.66 \\
\scriptsize{Sensor Effect Dom. Rand. 10k unaug. + 10k aug.}            &&&&& 48.53 &&&&& $\downarrow$2.48\\
\scriptsize{GTA\textit{Sim10k}$\rightarrow$KITTI 10k unaug. + 2k aug.} &&&&& 51.24 &&&&& $\uparrow$ 0.23\\ 
\scriptsize{GTA\textit{Sim10k}$\rightarrow$KITTI 10k unaug. + 5k aug.} &&&&& 51.95 &&&&& $\uparrow$ 0.94\\
\scriptsize{GTA\textit{Sim10k}$\rightarrow$KITTI 10k unaug. + 8k aug.} &&&&& 52.67 &&&&& $\uparrow$ \textbf{1.66}\\
\scriptsize{GTA\textit{Sim10k}$\rightarrow$KITTI 10k unaug. + 10k aug.}&&&&& 52.43 &&&&& $\uparrow$ 1.42\\
\hline
\end{tabular}
&  & &
%\hline
%\noalign{\smallskip}
\begin{tabular}{|l|llllllllll|}
%\hline
%\noalign{\smallskip}
\multicolumn{5}{c}{Training Dataset} & \multicolumn{5}{c}{Tested on Cityscapes}  \\
\hline
%\noalign{\smallskip}
Augmentation Method           &&&&& $AP_{Car}$ &&&&& \footnotesize{Gain} \\
%\noalign{\smallskip}
\hline
%\noalign{\smallskip}
GTA\textit{Sim10k} Baseline                                                  &&&&& 30.13          &&&&& \textemdash\\  
\scriptsize{Sensor Effect Dom. Rand. 10k unaug. + 2k aug.}                   &&&&& 33.64 &&&&& $\uparrow$3.51 \\ 
\scriptsize{Sensor Effect Dom. Rand. 10k unaug. + 5k aug.}                   &&&&& 34.56 &&&&& $\uparrow$4.43 \\
\scriptsize{Sensor Effect Dom. Rand. 10k unaug. + 8k aug.}                   &&&&& 34.24 &&&&& $\uparrow$4.11 \\
\scriptsize{Sensor Effect Dom. Rand. 10k unaug. + 10k aug.}                  &&&&& 34.70 &&&&& $\uparrow$4.57 \\
\scriptsize{GTA\textit{Sim10k}$\rightarrow$Cityscapes 10k unaug. + 2k aug.}  &&&&& 34.89 &&&&& $\uparrow$4.76 \\ 
\scriptsize{GTA\textit{Sim10k}$\rightarrow$Cityscapes 10k unaug. + 5k aug.}  &&&&& \textbf{35.48} &&&&& $\uparrow$ \textbf{5.35}\\
\scriptsize{GTA\textit{Sim10k}$\rightarrow$Cityscapes 10k unaug. + 8k aug.}  &&&&& 34.50 &&&&& $\uparrow$4.37 \\
\scriptsize{GTA\textit{Sim10k}$\rightarrow$Cityscapes 10k unaug. + 10k aug.} &&&&& 34.80 &&&&& $\uparrow$4.67 \\
%\multirow{2}{10em}{\small{Random Rotation, Scale, Transl., Crop}} &&&&& 55.11   &&&&& $\downarrow$ 3.14\\
%\noalign{\smallskip}
\hline
\end{tabular}
\end{tabular}
\end{center}
\end{table*}
\setlength{\tabcolsep}{1.4pt}
